A Large-scale Examination of "Socioeconomic" Fairness in Mobile Networks

Internet access is a special resource of which needs has become universal across the public whereas the service is operated in the private sector. Mobile Network Operators (MNOs) put efforts for management, planning, and optimization; however, they do not link such activities to socioeconomic fairness. In this paper, we make a first step towards understanding the relation between socioeconomic status of customers and network performance, and investigate potential discrimination in network deployment and management. The scope of our study spans various aspects, including urban geography, network resource deployment, data consumption, and device distribution. A novel methodology that enables a geo-socioeconomic perspective to mobile network is developed for the study. The results are based on an actual infrastructure in multiple cities, covering millions of users densely covering the socioeconomic scale. We report a thorough examination of the fairness status, its relationship with various structural factors, and potential class specific solutions.

==> sections/ACM-style/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> sections/ACM-style/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

==> sections/conclusion.tex <==
\section{Conclusion}
In this paper, we study the fairness of mobile network performance across the socioeconomic spectrum in three large cities of the UK, using data spanning over three years. Our work makes a first step towards understanding the mobile data usage from a socioeconomic perspective, as well as to investigate potential bias in MNO's network management and performance. To achieve this goal we devise a novel methodology leveraging continuous fine grained information about user mobility and data consumption, and  socioeconomic statistics. 

\textcolor{red}{Our examination of the fairness status reveals that all classes experience similar network performance. Associations between the socioeconomic class and performance measures (latency and packet-retransmission) are hardly found. The findings hold consistently throughout the studied periods and cities. The consistency is also examined across different seasons and the exceptional COVID-19 pandemic period.}

\textcolor{red}{A deeper investigation of the resource deployment, data consumption behaviors, and urban mobility has revealed a slightly different picture. Less network resources are deployed in the highest classes (e.g., IMD deciles 9 and 10 of London), and the number of devices served per sector is greater in those areas. The balance of the service quality is maintained nonetheless since the people of those classes consume less data. }

\textcolor{red}{As our work reflects on mobile networks from the socioeconomic perspective, novel implications are made. It demonstrates that the current network management practices is not leading to a bias against a particular class, which is important not only in the network measurement literature but also in the studies of social inequality. The details of the study also guides future resource deployment strategies tailored to different classes. The study also identifies a possible threat to fairness, and examines the potential impact of it based on urban geography and mobility patterns. The work serves as a basis for expanding the topic in multiple directions, for example, deeper investigation of the different data consumption behaviors of the classes, generalization to small cities and rural areas (of different demographics, geography, and network infrastructure), and application specific definitions of fairness and analysis. }

%As discussed, the results raise a number of important future research questions that could be of interest to the community; for example, whether the people of the highest classes are consuming less data as a consequence of relatively less radio sectors or not. While our speculation is that the data consumption is rather related to demographic and lifestyle factors than the availability of radio sectors, a longitudinal study of the data consumption behaviors and antenna deployment would be necessary to have a clear answer. In addition, there is a possibility of generalization of the  finding ``less consumption of the higher class and less sectors deployed''. The higher class could share important demographic and lifestyle factors, thereby showing similar data consumption behaviors, and less radio sectors might have been deployed accordingly. 
%similarly to~\cite{enrique-tool,enrique-cdr-girona}, 


%Our results show customers of different socioeconomic level use the network differently. Specifically, most deprived classes consume more data, while less deprivec customers are more mobile. From an MNO perspective, more resources are invested in area with lower socio-economic levels; as a consequence more people are connected and for longer time in least deprived areas. Despite the above trends, data consumption is fairly distributed accross sectors we do not observe any performance discrimination related to socio-economic factors. 
%Also, performance variability is related to geographical location of sectors. 
%\dpnote{Should we put all this?}
%This paper is only a first step towards a fully understanding of potential correlation and biases between network usage and management, and socio-economic factors.




==> sections/methodology_bck.tex <==
\section{Data \& Methodology}
\label{sec:methodology}
%\dpnote{Antennas and sectors are not unified now between the two part but we define sector in intro.}

In this paper we leverage two main data sources: i) passive traces collected from a large MNO from the United Kingdom (UK) with tens of millions of subscribers; ii) socioeconomic segmentation of the geographic space of London provided by the Index of Multiple Deprivation (IMD).\footnote{https://www.gov.uk/government/statistics/english-indices-of-deprivation-2015} 

We focus our analysis on London because it has various properties that are attractive for our study. Most importantly, the city hosts a diverse and large population of different classes and well connects the city segments. This allows a large-scale measurement study with people whose daily activity space largely overlap, and to analyze differences at a fine-grained level. 
%\spnote{what could be the benefits of zooming into one city? More ideas}
%- how the difference in the home area and daily mobility (despite sharing the same network infrastructure of the city) affects the usage of the network. 
%- allows to analyze differences at a finer-grained geographic areas.

We collect data for two distinct periods of two months each, \ie October-November 2018 and February-March 2019, in order to understand if our findings are consistent across time. As our findings hold for both periods, we report results of the latter only. In the following, we first detail the two datasets and then describe how we associate the users and sectors to the socioeconomic levels. We underline that the MNO under study does not track any socioeconomic status of its customers, while the UK government segment the countries in areas and report aggregate information to those. Hence, a methodology for combining the two datasets is required.

\subsection{Network \& mobility logs}
%\afnote{I would better articulate what the dataset contains, and the fact that carries the sector-ID}
%\spnote{Diego: Maybe we can address some of the IMC review points here? for example, the comment about how representative our data is}\dpnote{Done: please check if this is fine or need more.}
We analyze data collected at a \emph{transparent proxy} used by the MNO to optimize the entire mobile traffic and to log performance metrics about each user's transaction. The proxy handles traffic of all applications including both encrypted and non-encrypted flows. 
Specifically, for every flow, the transparent proxy stores the following layer 4 information: \emph{Round Trip Time (RTT)}, number of \emph{packet retransmission}, and \emph{total bytes transferred}. It also associates every flow to the sector where the user was located when the flow was active. 
These metrics are aggregated in two ways: first at the \emph{user} level,\ie across all transactions of a given user; second, at the \emph{sector} level, \ie across all transactions of all users performed in a given sector. Note that latency and packet retransmission are among the key performance metrics used to assess network quality. For instance, excessive latency (\ie round trip time) can hurt real time applications as streaming or VoIP, and generally impacts flow throughput. Also, a high number of packet re-transmissions may result in excessive network congestion, unacceptable delays and low throughput. The transparent proxy is located at the PGw/GGSN in the packet core, hence the metrics collected reflect the performance on the radio access (i.e., between the user device, and the egress point towards the Internet).
%Such aggregation is performed at different timescales. \spnote{?}

We also analyze information stored at the \emph{Mobility Management Entity (MME)} that keeps track of the radio sector where the subscribers are at any given time, thus providing temporally continuous location information. Note that, to respect the MNO dataset confidentiality policy, some results are normalized to avoid reporting raw values. %\spnote{Diego: what does this mean?} \dpnote{Better?}
In addition, the data used in the study did not include any personally identifiable information such as name or home address. We also did not link the data to other customer data (e.g., contract type and plans) since the MNO of our study does not manipulate the network performance depending on the type of contracts/plans. 

\subsection{Segmentation of space by socioeconomic spectrum}
The segmentation of the space is conducted by following the IMD metric, which is a statistical measure maintained by the UK government. The measure quantifies the relative deprivation for the areas in England at a very fine spatial granularity. This index combines seven distinct dimensions of deprivation: 1) Income deprivation, 2) Employment deprivation, 3) Health deprivation and disability, 4) Education, skills and training deprivation, 5) Crime, 6) Barriers to housing and services, and 7) Living environment deprivation. 

By combining the above seven dimensions, the overall IMD measure takes a wider interpretation of deprivation and looks into how much a group of people lack of resources of various kinds, not just income. As such, the IMD measure  has been used in studies of various domains (e.g., \cite{rivas2017exposure, mcgillion2017randomised}), considering it as an inclusive metric for the socioeconomic status. The combination of the seven dimensions is carefully defined in order to minimize cancellation effects; weights of the dimensions and the combination method is designed to prevent cases where a less deprivation of one dimension canceling out a deprivation of another dimension. Details of the combination method can be found at \cite{smith2015english}.

The index is maintained for all areas of the spatial division of England, called Lower-layer Super Output Areas (LSOAs). LSOAs are small areas divided to have similar population size and social homogeneity. An LSOA has an average of approximately 1,500 residents or 650 households. There are 32,844 LSOAa in England and 4,834 LSOAs in London. 

\begin{figure}[t]
\centering
  \includegraphics[width=0.85\linewidth]{Figs/methodology/LSOA_User_Dist.png}
%   	\vspace{-.4cm}
\caption{Number of LSOAs per decile in London
\label{fig:lsoa_cnt_decile}}
% 	\vspace{-.5cm}
\end{figure}

Based on the deprivation score, a ranking is made with all LSOAs in England. 
Beside punctual scores, the government publishes also \emph{deciles}, i.e., it splits the 32,844 LSOAs into 10 equal-sized groups, from the most deprived (index 1) to the least deprived (index 10). The LSOAs in decile 1 fall within the most deprived 10\% nationally and the LSOAs in decile 10 fall within the least deprived 10\%. The skyblue bars of Figure \ref{fig:lsoa_cnt_decile} shows the distribution of LSOAs in London over the IMD deciles. It shows that the LSOAs of both extremes (1 and 10) are significantly less than those of others in London, and there are relatively more number of LSOAs of the lower deciles (e.g., decile 2, 3, and 4). 

As the latest IMD census was conducted in 2015, there is a time gap between the network logs and the IMD data. In order to examine the validity of combining the two datasets, we analyze how dynamic the IMD deciles are over time. We compare the IMD deciles of the last three censuses (2007, 2010, and 2015), and observe very little difference: between the census of 2010 and 2015, the kendall rank correlation of the IMD deciles is 0.89; between 2007 and 2015, 0.84. We thus assume that the IMD deciles in 2019 would remain very close to the ones 2015 dataset. 

\subsection{Segmentation of users by socioeconomic spectrum}
The government census data provides aggregation based on the declared people residence address. Hence, to combine such information with the MNO dataset, we need to identify in which LSOA the MNO customers seem to be living based on their mobility patterns.
%Based on the segmentation of the space of London, the users are segmented by identifying their home LSOAs from their mobility traces. 
While there are many methods for identifying home of people from mobility traces, they commonly aim at finding regularity during night time and/or weekends (\cite{kung2014exploring,bojic2015choosing}). Likewise, we develop a method for home sector detection specific to our dataset with the same intuition. 

As mentioned, MME has temporally continuous traces. We go through the data of all the days throughout a month for each device, and approach to identify the ones who connects to the same sector at night time (midnight - 8AM) for substantial number of days. The method first identifies the set of sectors to which a device connects during the night time (midnight - 8AM) of every day. To ensure that the device is staying in an area during the time window, we employ the radius of gyration to estimate the spatial deviation of a device and filter out the days when the estimated radius is larger than 2km.\footnote{The threshold is a conservative value of the area covered by a sector.} Finally, the method identifies the home sector of a device as the one which was connected at least two weeks during a month, and has the maximum connection duration. The devices that do not have a home sector that satisfies the criteria are excluded from the study. 

This home detection method identifies the home sector for 1.2M devices, and the sample user set has at least 27k residents for every decile. The identified homes are widely distributed across the city: the detected home antennas' coverage overlap with 4,813 LSOAs out of 4,835. The purple bars of Figure \ref{fig:lsoa_cnt_decile} shows the distribution of the people identified as London residents. The similarity of the distribution to that of the LSOAs over the IMD decile supports the reliability of our sample and the home detection method.

\iffalse

\begin{figure*}[h]
\centering
\subfigure[User data consumption across IMDs]{
	\includegraphics[width=0.3\linewidth,height=0.22\linewidth]{Figs/Usage/bytes_IMD.png}\label{fig:bytes-imd}
	}
\subfigure[Ratio of data consumed via 4G]{
	\includegraphics[width=0.3\linewidth,height=0.22\linewidth]{Figs/Usage/4G_consumption_ratio.png}\label{ratio4g-imd}
	}
\subfigure[Pairwise visits between IMD deciles]{
	\includegraphics[width=0.36\linewidth,height=0.25\linewidth]{Figs/Usage/Lon_Jan_1h_all.png}\label{fig:mob_mtx}
	}
	\vspace{-.4cm}
	\caption{Aggregated user level analysis.}
	\vspace{-.4cm}
\end{figure*}

\fi

%\subsection{Scope and limitations}
%\dpnote{Do not think we need this section at this point. We acknowledge in conclusion what we plan to do as future work. Also better to avoid saying anything about M2M. So would remove.}
%Only one city. Only some metrics available. Potential biases due to our dataset.
%We have a mixture of M2M and actual users (wearables, smartphones): M2M generate little traffic and is about 20\% OR do filtering or breakdown.







==> sections/performance.tex <==
\section{Performance Metrics}

\begin{figure}[t]
\centering
\subfigure[Avg. packet retran. frequency of TCP sessions]{
	\includegraphics[width=0.7\linewidth]{Figs/Usage/User_Pktret_IMD.png}\label{fig:quality_user_imd_rtx}
	}
\subfigure[Avg. latency of sessions]{
	\includegraphics[width=0.7\linewidth]{Figs/Usage/User_Lat_IMD.png}\label{fig:quality_user_imd_latency}
	}
	\vspace{-.4cm}
	\caption{Aggregated user level performance metrics.}
	\vspace{-.5cm}
\end{figure}

%\dpnote{We use average for users and median for sector by mistake. We will have to normalize to different values. We will then fix in CR, no time now.}
We now investigate whether the trend observed in the previous section have an impact on the user and sector performance. We focus on 4G only, as we observed in Sec.~\ref{sec:usage} that almost all consumption is made via 4G. Results are averaged over two months, and reported for weekdays only (though not reported, the reported findings also hold for weekends).

%We extend our analysis by delving into the QoE of individual users. This analysis provides a different view from the above space-based (\spnote{or sector-based?}) analyses as people make connections in different sectors depending on their daily mobility.
%For every user identified as a resident of London, we track all the connections in London throughout the studied period. As we are interested in potential socio-econmic biases, the analysis is focused on answering the follwoing two primary questions: first, if socio-economic status has an impact on 4G technology access; second, if the connection quality of users show an association with their socio-economic status. Figure XX shows the daily-average time (in seconds) of users' devices staying connected to 4G technology. The distributions do not show much difference among the IMD deciles, suggesting weak support for the socio-economic bias in 4G technology access. Across all IMD deciles, majority of the people are connected via 4G technology between XXX seconds and YYY seconds \spnote{maybe a linear regression or ANOVA to run a significance test}. 

\noindent\textbf{User level performance - }
%\dpnote{If anova is not conclusive we may say that we do not observe any difference.}
We employ two metrics: packet retransmission frequency and round trip time. Fig~\ref{fig:quality_user_imd_rtx} reports the daily average packet retransmission frequency of a user (\ie number of packet re-transmitted over total number of packets of a flow, averaged across all flows of a day), and Fig.~\ref{fig:quality_user_imd_latency} the daily average  latency (\ie average RTT experienced by the user, averaged across all  flows of a day). Results are normalized over the highest 90-percentile to preserve MNO confidentiality. 

Overall, we do not see a clear association between the performance metrics and socioeconomic status. We only observe a slight association between the packet retransmission frequency and the IMD deciles: the median, 70 and 90 percentiles slightly decrease along  the IMD deciles. One-way ANOVA confirms the difference (F(9, 997255) = 177.94, \textit{p} $<$ .01) and the post-hoc analysis shows that deciles 7, 8, 9, 10 have lower retransmission frequency than the deciles from 1 to 5. The latency, on the other hand, do not show a consistent tendency along the IMD decile. 


% FOR REFERENCE: For quality analysis, We employed two metrics, packet drop frequency per TCP session and round trip time (Figure \ref{fig:quality_user_imd}). One speculation made based on the above observation was that the lower data consumption of the higher class may have been affected by lower connection quality. However, we do not observe clear signs of lower quality. In fact, we observe a decreasing tendency of the packet drop frequency over the IMD deciles. The difference is analyzed in the same way (one-way ANOVA, F(9, 997255) = 177.94, \textit{p} $<$ .01) and the post-hoc analysis showed that deciles 7, 8, 9, 10 have lower drop frequency than the deciles from 1 to 5. The latency, on the other hand, did not show a consistent tendency along the IMD decile. 

%\noindent\textbf{Sector level performance - }
%Fig~\ref{fig:quality_sector_imd} reports the daily average packet retransmission frequency and minimum latency (see above), aggregated at sector level. The most striking result is that we do not observe a clear trend between the performance metrics and socio-economic level of different areas.
\noindent\textbf{Sector level performance - }
The results are similar for sector level performance (not shown due to the lack of space). Only a slight association between packet retransmission frequency and IMD deciles is found: one-way ANOVA confirms the existence of a difference among deciles (F(9, 6068) = 8.03, \textit{p} $>$ .01), and the post-hoc analysis shows that deciles  8, 9, 10 have a lower retransmission frequency than the deciles from 1 to 3. On the other hand, no significant difference is found for the latency across IMDs. 

The lack of a clear trend across the IMD deciles indicates that there are other factors rather than the socioeconomic status of the areas that creates the variance of sector performance. To take a step further, we attempt to analyze the under-performing sectors from a geographical perspective. 
First, we verify if the under-performing sectors are consistent over time. For every day, we identify the sectors whose latency/packet retransmission frequency is within 75 and 90 percentile as the reference of the under-performing set of that day. We then compute the degree of overlap of those sets between every pair of the days of the study period using the Jaccard index \footnote{https://en.wikipedia.org/wiki/Jaccard\_index}. While the results are omitted due to the lack of space, the distribution of the Jaccard index confirmed that for any pair of days within the studied period, more than half of the sectors of the under-performing set overlaps. 

%In order to understand the high performance variability (\ie 90-percentile values) we focus on sectors whose latency/packet retransmission frequency is within 75 and 90 percentile for at least one day over the two months (defined in the following as problematic sectors). Specifically, we compute the Jaccard similarity index between the set of problematic sectors of every pairs of days of the two months. Results reported in Fig.~\ref{fig:jaccard-space} for packet retramsmission frequency only as they also hold for latency. We observe a Jaccard index fairly concentrated around 0.4 across all IMD deciles.  A Jaccard index value around 0.4 means that on given a day, among the set of sectors that don't perform well, half of them will not perform well in another day at least. This highlight such sectors are \emph{hot-spots}~\cite{hotornot}, as their performance issues are consistent across time\dpnote{Should we say something about hotspot duration from hotornot?}.

We then mapped the frequent under-performing sectors and observed that they are mostly located in the city center in popular neighborhoods (\ie 80\%), with a few exception of them being located near the boundary of the city (\ie 20\%). It follows performance issues are mostly related to a large number of people connected to sectors, or bad coverage. 

\noindent\textbf{Takeaway: }\emph{Despite the results of previous sections highlighting some correlations between network usage \& management and socio-economic levels, we do not see a clear correlation between network level performance and socioeconomic status. A follow-up analysis suggests that the performance variance is due to the presence of hot-spots that are related to geographical locations of different sectors rather than socio-economic factors.}

==> sections/space.tex <==
\section{Sector level analysis}
%\dpnote{Need to normalize results for confidentiality. HIGH PRIORITY}
%\dpnote{Add sector KPIs analysis? Look at hotspots. LOW PRIORITY}
%\dpnote{Add hour of day analysis. LOW PRIORITY}
%As we observed a significant correlation between socio-economic level of customers and their network usage patterns, we now investigate how this interplays with the MNOs sector management policy based on KPIs. 
%Part of previous story
We expand the study by taking a sector level perspective to the data. This allows to explore potential correlations between socioeconomic status and sector management policies, and also to gain insights on the structural reasons behind user-level observations made in the previous section. Results are averaged over two months and reported for weekdays only as they hold for weekends as well. We focus on 4G due to its dominance in terms of data consumption (cf. Sec.~\ref{sec:usage}).

\begin{figure}[t]
\centering
	\includegraphics[width=0.8\linewidth]{Figs/Sector/byte-exchanged-sector.pdf}
	\vspace{-.4cm}
	\caption{Avg number of bytes per sector.}\label{fig:bytes-sectors-imd}
	\vspace{-.6cm}
\end{figure}

\noindent\textbf{Sector distribution across IMDs - }
We first look at the distribution of numbers of sectors per LSOA across the IMD deciles in Fig.~\ref{fig:sector-imd}. 
%Recall that we only focus on 4G antennas due to its dominance in terms of data consumption.
The main striking results is that the distribution of sectors is similar for the first 7-8 IMD deciles, with a drop in the number of sector per LSOAs for IMD 9-10. LSOAs belonging to the former group (\ie lower class areas), have 3 sectors located within the LSOA in the median case. Differently, most LSOAs belonging to last IMD deciles (\ie higher class areas) do not have an antenna of a sector located within the LSOA and users are connected via antennas located in nearby areas.

\noindent\textbf{Sector load across IMDs - }
We then move on to examining possible unbalance in terms of sector load. The sector load is estimated in three ways: first, the cumulated time per day, which is defined as the total amount of time spent by all devices (\ie sum across devices) connecting to a sector in a day; second, the number of devices per day, which is the count of devices connecting to a sector in a day; third, the average number of bytes transferred in a day. 

Fig. ~\ref{fig:time-density-breakdown} plots the cumulated time load for an average case of each IMD decile, dissecting the load created by \emph{residents} and \emph{non-residents}. We see an increase of load for the higher class; for instance the median time load of IMD 10 is almost double the one of IMD 1. Separating the cumulated time between residents vs. non-residents further reveals that the time load is coming from the devices of the residents. Our interpretation is that the sectors near higher class areas handle more residents as there are fewer sector near those areas (cf. Fig.~\ref{fig:sector-imd}). This is supported by Fig.~\ref{fig:device-density-breakdown}, showing that there are greater number of residents' devices  covered by a sector in higher class areas. 

Another observation can be made by putting Fig.~\ref{fig:device-density-breakdown} together with Fig. ~\ref{fig:time-density-breakdown}. Although the non-residents' devices dominate (>80\%) the overall number of devices for all deciles according to Fig.~\ref{fig:device-density-breakdown}, the proportion of the cumulated time of them is far less in contrast to their dominance. This indicates that the actual load of the sectors is likely to depend more on the load of the nearby residents than non-residents.

%One-way ANOVA\dpnote{\footnote{ADD reference or explain anova}} shows that differences in the number of devices are observed among the deciles (F(9, 12110) = 6.37, \textit{p} $<$ .01), and the post-hoc analysis confirm that the deciles 9 and 10 show significant difference from all the deciles below. 

%In order to understand the first trend, we divide the customers into \emph{residents} and \emph{non-residents} in Fig.~\ref{fig:device-time-density-breakdown} for an average 4G sector in a weekday and weekend day. We observe the time load (left axis) related to residents  of  IMD deciles 9-10 is higher than in lower IMD areas, \eg the resident sector time load of IMD 10 is more than double than the one of IMD 1.  As shown in the figure, this is due to the number of resident devices (right axis) connected to each sector that increases with IMD deciles as the number of sector per LSOA decreases (cf. Fig.~\ref{fig:sector-imd}).

%We then report in Fig.~\ref{fig:time-density} the daily time load of a sector, that is defined as the total amount of time spent by all devices (\ie sum across devices) in a day in a sector of a given LSOA. Results are normalized over \dpnote{XXX}, averaged over two months and reported for 3G and 4G. Although not shown, these results are consistent for weekends and weekdays. For 4G we observe the time load increases with the IMD deciles; for instance the median time load of IMD 10 is almost double the one of IMD 1. Conversely, we observe the reverse trend for 3G; for instance we notice a 40\% decrease in time load from IMD decile 1 to IMD decile 10. \dpnote{Not sure how to explain this last. Maybe remove?} 


%\afnote{The plot is really hard to read :(}
%In order to understand the first trend, we divide the customers into \emph{residents} and \emph{non-residents} in Fig.~\ref{fig:device-time-density-breakdown} for an average 4G sector in a weekday and weekend day. We observe the time load (left axis) related to residents  of  IMD deciles 9-10 is higher than in lower IMD areas, \eg the resident sector time load of IMD 10 is more than double than the one of IMD 1.  
%As shown in the figure, this is due to the number of resident devices (right axis) connected to each sector that increases with IMD deciles as the number of sector per LSOA decreases (cf. Fig.~\ref{fig:sector-imd}). For instance, the number of residents connected to a sector of IMD decile 10 is 80\% higher than in a sector of IMD decile 1. One-way ANOVA analysis shows that differences are observed among the deciles (F(9, 12110) = 6.37, \textit{p} $<$ .01), and the post-hoc analysis confirm that the deciles 9 and 10 show significant difference from all the deciles below. 

%Fig.~\ref{fig:device-time-density-breakdown} also shows that more distinct devices are observed during weekdays especially for IMD deciles 4-6. This is mostly due to the non-residents that work in the city and live outside London.  However, the time load is fairly similar between weekend and weekdays. This is due to the significant contribution of residents to the time load, but also to the longer sejourn times of non-resident during weekends (\eg tourists, family visitors).

%\noindent\textbf{Bytes distribution across IMDs - }
Despite the differences in the cumulated time load and the number of devices, we do not see a clear unbalance in the traffic (avg. bytes per day) served by the sectors. Fig.~\ref{fig:bytes-sectors-imd} (data exchanged per sector is normalized over the highest 90-percentile to preserve MNO confidentiality) shows that the medians are fairly close among all deciles. The median is even slightly less for the higher class although the sectors of such areas handle more number of devices. This is consistent to our user-level observation that residents of higher class areas consume less data. However, the difference is marginal and we do not see a clear trend: one-way ANOVA shows that there is a difference among the deciles (F(9, 14064) = 6.14, \textit{p} $<$ .01); however, the post-hoc analysis only confirms difference for occasional cases (e.g., difference of decile 10 from deciles 1-5, deciles 8 from decile 2-4) rather than a consistent trend. 
%Finally, we investigate the amount of data exchanged on a day on average per LSOA in both 3G and 4G in Fig.~\ref{fig:bytes-sectors-imd}. 
%Although not shown, these results are consistent for weekends and weekdays. 
%We observe the amount of data exchanged over 3G and 4G decreases with the IMD deciles. Despite there are less antennas per LSOA and sectors have an higher time load in higher IMDs (\ie richer areas), less data is consumed in these areas. This is mostly due to the fact that residents of these area consumes less data with respect to customers of lower IMD deciles (cf. Fig.~\ref{sec:usage}). 

\noindent\textbf{Takeaway: }\emph{Less resources are invested in areas with higher IMD deciles. As a consequence, sectors of higher class areas are more loaded in terms of connected devices and time, and this is mostly due to residents of such areas. However, as these customers generate less traffic, we do not see a strong unbalance in terms of the overall traffic across the socioeconomic spectrum.}

==> sections/usage.tex <==
\section{User Data Network Usage}
\label{sec:usage}

%\dpnote{Need to normalize results for confidentiality. HIGH PRIORITY}

We start our analysis by taking an overview of the individuals' mobile network usage with respect to their socioeconomic status. The overall data consumption and the mobility in the connections are explored to search for possible signs of biases. Results are averaged over two months and reported for weekdays only as they hold for weekend as well.

\noindent\textbf{User Data Consumption - }
%\afnote{I would suggest a different flow for the section: mobility first (gyration+matrix) and then usage. Because you can congecture that the more static nature of people can lead to higher usage. It would have been nice to check the timeonrat features too. Meaning, if you assume that more reach people leave outside, it is possible that they connect less to 4G because of coverage (which is different from data usage in 4G that you have here)}
We analyze the amount of mobile data consumption among IMD deciles in Fig.~\ref{fig:bytes-imd}. Specifically, we report the percentage of users with low consumption (\ie less than 10~MB per month - the 10-percentile of customers when ranked by data usage) and high consumption (\ie more that 5~GB per month - the 90-percentile of customers when ranked by data consumption) across IMDs. Note that customers generating more than 5~GB of traffic account for 50\% of the overall data traffic. We first observe  that the percentage of the low consumption group is small and similar across all classes. Interestingly, the high consumption group is much larger in the lower deciles. For instance, the high consumption group of the lowest decile is double of that of the highest decile. 

While Fig.~\ref{fig:bytes-imd} shows the groups of both extreme, the mean consumption of the deciles are also found to be different. One-way ANOVA \cite{fisher2006statistical} confirms the existence of a significant difference (F(9, 997255) = 177.94, \textit{p} $<$ .01)), and a post-hoc analysis (Tukey's HSD\footnote{\url{https://en.wikipedia.org/wiki/Tukey\%27s_range_test}}) shows that the mean consumption of the deciles 7, 8, 9, 10 are lower than that of all the deciles from 1 to 6.

%Interestingly, our measurement of the overall data consumption (daily average) across the socioeconomic spectrum reveals a slight but statistically significant trend showing that higher class people consume less mobile data. A one-way ANOVA confirms the existence of a difference (F(9, 997255) = 177.94, \textit{p} $<$ .01)), and a post-hoc analysis (Tukey's HSD) shows that the mean byte consumption of the deciles 7, 8, 9, 10 are lower than that of all the deciles from 1 to 6. As this overall trend is not sharp as mentioned, we took a step further and observed that a strong tendency is observed when focusing on the heavy consumers (Figure X).

%The large variance among the people of the same decile is expected as different people have different phone usage habits \spnote{cite?}. 


%Figure \ref{fig:bytes-imd} depicts the overall data consumption (daily average) across the socioeconomic spectrum. 
%The large variance among the people of the same decile is expected as different people have different phone usage habits \spnote{cite?}. 
%However, an interesting trend is observed toward the higher deciles: the richer class consumes less mobile data. 
%The difference of the consumption is significant (one-way ANOVA, F(9, 997255) = 177.94, \textit{p} $<$ .01). A post-hoc analysis (Tukey's HSD) shows that the mean byte consumption of the deciles 7, 8, 9, 10 are lower from all those of the deciles from 1 to 6.
%\afnote{...I think this effect was clearer in the plot of the other paper}

\begin{figure}[t]
\centering
	\includegraphics[width=0.8\linewidth]{Figs/Usage/avg_gyration.png}
	\vspace{-.2cm}
	\caption{Average gyration across IMD deciles}\label{fig:gyration-imd}
	\vspace{-0.5cm}
\end{figure}

\noindent\textbf{Technology Usage - }
We also brake down the consumption via technology (4G vs. 3G) to analyze if the socioeconomic status has an association with 4G technology access. For each individual user, we compute the ratio of data consumption made via 4G to all consumption. The result (Figure \ref{ratio4g-imd}) shows that most of the consumption is made via 4G regardless of the socioeconomic status. For all the IMD deciles, the variance within the decile is also small, indicating that all the users are on 4G in general. Since most of the data consumption is made via 4G, we focus on the 4G connections in the presentation of our following analyses.

%second, the ratio is slightly less for the higher class relative to the others. The difference of the ratio among the IMD deciles is significant (one-way ANOVA, F(9, 997255) = 80.75, \textit{p} $<$ .01). A post-hoc analysis (Tukey's HSD) shows that the mean byte consumption of the deciles 7, 8, 9, 10 are lower from all those of the deciles from 1 to 6. 
%\afnote{by how much? is this a significant difference?}

%Since most of the data consumption is made via 4G, we focus on the 4G connections in the presentation of our following analyses. For quality analysis, We employed two metrics, packet drop frequency per TCP session and round trip time (Figure \ref{fig:quality_user_imd}). One speculation made based on the above observation was that the lower data consumption of the higher class may have been affected by lower connection quality. However, we do not observe clear signs of lower quality. In fact, we observe a decreasing tendency of the packet drop frequency over the IMD deciles. The difference is analyzed in the same way (one-way ANOVA, F(9, 997255) = 177.94, \textit{p} $<$ .01) and the post-hoc analysis showed that deciles 7, 8, 9, 10 have lower drop frequency than the deciles from 1 to 5. 

%The latency, on the other hand, did not show a consistent tendency along the IMD decile. 

%We first consider the amount of devices and traffic used by customers of different socioeconomic levels. Then we investigate their mobility traffic patterns.



\begin{figure*}[t]
\centering
\subfigure[Distribution of number of sectors per LSOA.]{
	\includegraphics[width=0.3\linewidth]{Figs/Sector/Sector_IMD.png}\label{fig:sector-imd}
	}
\subfigure[Cumulated time load of an average sector.]{
	\includegraphics[width=0.3\linewidth]{Figs/Sector/time-density-breakdown.pdf}\label{fig:time-density-breakdown}
	}
\subfigure[Percentage of resident devices per day of an average sector. Raw values on top of bars.]{
	\includegraphics[width=0.3\linewidth]{Figs/Sector/device-perc-density-breakdown.pdf}\label{fig:device-density-breakdown}
	}
	\vspace{-.4cm}
	\caption{Aggregated sector level analysis.}
	\vspace{-.4cm}
\end{figure*}




%Our study revealed that the degree of segregation is different among the classes, and that the higher and middle classes tend to reach out more diverse areas than the lower class. We believe that these observations can be connected to and partly explained by the general relationship between mobility and socioeconomic status. 

\noindent\textbf{User Mobility - }
We also explore the mobility of individuals to better understand from where people connect, and how that vary across the socioeconomic spectrum. We attempt to measure the diversity of the sectors that each individual connects to by computing the radius of gyration. The gyration is a weighted measure based on the location of the connected sectors and the aggregated duration of the connections, and can be interpreted as the `typical distance traveled in a day.' Figure~\ref{fig:gyration-imd} depicts the distribution of the gyration across the IMD deciles. While the body of the distribution of all the deciles falls in the range of 1-10~km, the median values present a clear trend of richer people showing greater mobility. This is consistent to the literature in geography \cite{7363835, dodson2004transport}, which finds that the  deprived classes exhibits less mobility, possibly due to cost burden and disadvantage in terms of transportation access.

%\noindent\textbf{Takeaway:}\emph{Customers of higher IMD levels have a larger number of devices connected to the network and are more mobile than customers of lower IMD levels. Conversely, customers of lower IMD classes generate more data traffic.}

We further analyze from which IMD decile people are connecting when they are not in their home areas. We construct a $10\times10$ matrix where each row and column indicate the decile index of the home and the visited destination, respectively. Each row aggregates the frequency of visits made to the 10 deciles. The matrix is normalized by rows (divide-by-sum) considering the uneven number of LSOAs per decile in London. The result is shown in Figure \ref{fig:mob_mtx}, where the rows can be read as "going to" and each cell as the percentage of the visits made to the corresponding decile. The color is darker for higher percentage. The result shows that the lower class (deciles below 5) tend to visit similar areas in terms of the socioeconomic status whereas the mobility of the above classes is more dispersed over diverse areas. A consequent implication that can be obtained from the results is that the complexity of understanding the experience of the network quality would be different depending on the socioeconomic class: the diversity of the connected sectors greatly varies among the classes.

\noindent\textbf{Takeaway: } \emph{Proportion of the heavy consumers (\ie people consuming more than 5~GB per month, accounting for 50\% of the overall traffic) is larger in lower classes. On the other hand, less deprived customers tend to be more mobile and they connect from more diverse areas, both in terms of physical locations and socioeconomic status.}



